Do Drug Consumption Rooms Reduce Drug-Related Hospitalizations? Evidence from Switzerland

This paper estimates the causal effect of drug consumption room (DCR) openings on drug-related hospitalizations in Switzerland. I exploit the staggered introduction of DCRs across Swiss cities between 1998 and 2022, using individual-level hospital records and a difference-in-differences estimator. DCR openings reduce drug-related hospitalization rates by roughly 35\% within 5 km of a facility. The reduction is most pronounced for fatal outcomes, which fall by 35\% while narcotics poisoning hospitalizations rise by a comparable amount, consistent with DCRs converting potentially fatal overdoses into non-fatal hospitalizations. Mental and behavioral disorder hospitalizations decline by 32\% while estimates for Hepatitis and HIV are imprecise. The findings support the role of DCRs as an effective harm reduction strategy.

==> tables/att_summary_1km.tex <==
% latex table generated in R 4.5.1 by xtable 1.8-4 package
% Fri Aug 15 08:11:41 2025
\begin{table}[H]
\centering
\begin{tabular}{rrrrrr}
  \hline
Group & Time & ATT & SE & Lower\_CI & Upper\_CI \\ 
  \hline
2001 & 1999 & -0.00 & 0.01 & -0.02 & 0.02 \\ 
  2001 & 2000 & 0.00 & 0.00 & -0.00 & 0.01 \\ 
  2001 & 2001 & -0.00 & 0.00 & -0.01 & 0.01 \\ 
  2001 & 2002 & 0.00 & 0.00 & -0.01 & 0.01 \\ 
  2001 & 2003 & -0.00 & 0.00 & -0.01 & 0.01 \\ 
  2001 & 2004 & -0.01 & 0.00 & -0.02 & 0.01 \\ 
  2001 & 2005 & -0.00 & 0.00 & -0.02 & 0.01 \\ 
  2001 & 2006 & 0.01 & 0.01 & -0.01 & 0.03 \\ 
  2001 & 2007 & -0.00 & 0.01 & -0.02 & 0.01 \\ 
  2001 & 2008 & 0.02 & 0.01 & 0.00 & 0.03 \\ 
  2001 & 2009 & 0.03 & 0.02 & -0.02 & 0.09 \\ 
  2001 & 2010 & 0.03 & 0.02 & -0.02 & 0.08 \\ 
  2001 & 2011 & 0.03 & 0.01 & -0.01 & 0.06 \\ 
  2001 & 2012 & 0.02 & 0.01 & -0.00 & 0.04 \\ 
  2001 & 2013 & 0.02 & 0.01 & -0.01 & 0.05 \\ 
  2001 & 2014 & 0.01 & 0.00 & 0.00 & 0.02 \\ 
  2001 & 2015 & 0.01 & 0.00 & 0.00 & 0.02 \\ 
  2001 & 2016 & 0.01 & 0.00 & -0.00 & 0.02 \\ 
  2001 & 2017 & 0.01 & 0.00 & -0.01 & 0.02 \\ 
  2001 & 2018 & 0.01 & 0.00 & -0.00 & 0.02 \\ 
  2001 & 2019 & 0.01 & 0.00 & -0.01 & 0.02 \\ 
  2001 & 2020 & 0.00 & 0.00 & -0.01 & 0.02 \\ 
  2001 & 2021 & 0.00 & 0.00 & -0.01 & 0.01 \\ 
  2001 & 2022 & 0.01 & 0.00 & -0.00 & 0.02 \\ 
  2013 & 1999 & -0.01 & 0.00 & -0.02 & -0.00 \\ 
  2013 & 2000 & 0.00 & 0.00 & -0.00 & 0.00 \\ 
  2013 & 2001 & -0.01 & 0.00 & -0.02 & -0.00 \\ 
  2013 & 2002 & 0.01 & 0.00 & 0.00 & 0.02 \\ 
  2013 & 2003 & 0.00 & 0.00 & -0.00 & 0.01 \\ 
  2013 & 2004 & 0.00 & 0.00 & -0.00 & 0.00 \\ 
  2013 & 2005 & 0.00 & 0.00 & -0.01 & 0.01 \\ 
  2013 & 2006 & -0.00 & 0.00 & -0.00 & 0.00 \\ 
  2013 & 2007 & 0.00 & 0.00 & -0.01 & 0.01 \\ 
  2013 & 2008 & -0.00 & 0.00 & -0.02 & 0.01 \\ 
  2013 & 2009 & 0.00 & 0.00 & -0.00 & 0.01 \\ 
  2013 & 2010 & -0.00 & 0.00 & -0.01 & 0.01 \\ 
  2013 & 2011 & 0.00 & 0.00 & -0.00 & 0.01 \\ 
  2013 & 2012 & -0.00 & 0.00 & -0.01 & 0.00 \\ 
  2013 & 2013 & -0.00 & 0.00 & -0.01 & 0.00 \\ 
  2013 & 2014 & -0.00 & 0.00 & -0.01 & 0.00 \\ 
  2013 & 2015 & -0.00 & 0.00 & -0.00 & -0.00 \\ 
  2013 & 2016 & -0.00 & 0.00 & -0.00 & 0.00 \\ 
  2013 & 2017 & -0.00 & 0.00 & -0.01 & -0.00 \\ 
  2013 & 2018 & -0.00 & 0.00 & -0.01 & 0.00 \\ 
  2013 & 2019 & -0.01 & 0.00 & -0.01 & -0.00 \\ 
  2013 & 2020 & -0.00 & 0.00 & -0.01 & -0.00 \\ 
  2013 & 2021 & -0.00 & 0.00 & -0.01 & 0.00 \\ 
  2013 & 2022 & -0.00 & 0.00 & -0.01 & 0.00 \\ 
  2018 & 1999 & 0.00 & 0.00 & -0.00 & 0.00 \\ 
  2018 & 2000 & -0.00 & 0.00 & -0.00 & 0.00 \\ 
  2018 & 2001 & 0.00 & 0.00 & -0.00 & 0.00 \\ 
  2018 & 2002 & 0.00 & 0.00 & -0.00 & 0.00 \\ 
  2018 & 2003 & 0.00 & 0.00 & -0.00 & 0.00 \\ 
  2018 & 2004 & 0.00 & 0.00 & -0.00 & 0.00 \\ 
  2018 & 2005 & -0.00 & 0.00 & -0.00 & 0.00 \\ 
  2018 & 2006 & 0.00 & 0.00 & -0.00 & 0.00 \\ 
  2018 & 2007 & -0.00 & 0.00 & -0.00 & 0.00 \\ 
  2018 & 2008 & 0.01 & 0.01 & -0.01 & 0.03 \\ 
  2018 & 2009 & 0.01 & 0.00 & 0.00 & 0.01 \\ 
  2018 & 2010 & -0.00 & 0.00 & -0.01 & 0.00 \\ 
  2018 & 2011 & 0.00 & 0.00 & -0.00 & 0.00 \\ 
  2018 & 2012 & 0.00 & 0.00 & -0.00 & 0.00 \\ 
  2018 & 2013 & -0.00 & 0.00 & -0.01 & 0.00 \\ 
  2018 & 2014 & -0.00 & 0.00 & -0.01 & -0.00 \\ 
  2018 & 2015 & -0.00 & 0.00 & -0.01 & 0.00 \\ 
  2018 & 2016 & -0.00 & 0.00 & -0.00 & 0.00 \\ 
  2018 & 2017 & 0.00 & 0.00 & -0.00 & 0.01 \\ 
  2018 & 2018 & 0.01 & 0.00 & 0.00 & 0.01 \\ 
  2018 & 2019 & 0.01 & 0.00 & 0.00 & 0.01 \\ 
  2018 & 2020 & 0.00 & 0.00 & -0.00 & 0.01 \\ 
  2018 & 2021 & 0.01 & 0.00 & 0.00 & 0.01 \\ 
  2018 & 2022 & 0.01 & 0.00 & -0.00 & 0.01 \\ 
   \hline
\end{tabular}
\caption{Group-Time ATT Estimates (1km buffer)} 
\label{tab:att_1km}
\end{table}

==> tables/master_balance_pretty.tex <==
\begin{table}[H]
\caption{Balance table across rurality, education, socio-professional, demographics, and age shares and absolute standardized differences (treated vs control MedStat regions).}
\centering
\tiny
\begin{tabular}{lccc}
\toprule
 & \textbf{Treated Mean} & \textbf{Control Mean} & \textbf{Abs. Std. diff.} \\
\midrule
\textbf{Rurality} \\
\quad Intermediate & 0.05 & 0.24 & 0.56 \\
\quad Rural & 0.00 & 0.33 & 0.99 \\
\quad Urban & 0.95 & 0.42 & 1.36 \\
\addlinespace
\textbf{Education} \\
\quad No education & 0.04 & 0.04 & 0.00 \\
\quad Mandatory school & 0.17 & 0.20 & 0.06 \\
\quad Apprenticeship & 0.27 & 0.31 & 0.09 \\
\quad Maturity & 0.07 & 0.04 & 0.14 \\
\quad University & 0.10 & 0.04 & 0.20 \\
\quad Low education & 0.21 & 0.23 & 0.06 \\
\quad Medium education & 0.34 & 0.35 & 0.02 \\
\quad High education & 0.10 & 0.04 & 0.20 \\
\addlinespace
\textbf{Socio-professional} \\
\quad Managers & 0.01 & 0.01 & 0.01 \\
\quad Liberal professions & 0.01 & 0.01 & 0.04 \\
\quad Other independents & 0.04 & 0.05 & 0.07 \\
\quad Intellectual/exec. & 0.06 & 0.04 & 0.10 \\
\quad Intermediate prof. & 0.08 & 0.08 & 0.01 \\
\quad Qualified non-manual & 0.10 & 0.10 & 0.00 \\
\quad Qualified manual & 0.03 & 0.04 & 0.09 \\
\quad Unqualified workers & 0.06 & 0.06 & 0.03 \\
\quad Active (unattributed) & 0.14 & 0.13 & 0.03 \\
\quad Unemployed & 0.03 & 0.02 & 0.08 \\
\quad Inactive & 0.32 & 0.28 & 0.07 \\
\addlinespace
\textbf{Demographics} \\
\quad Female share & 0.53 & 0.51 & 0.04 \\
\quad Swiss share & 0.73 & 0.82 & 0.23 \\
\addlinespace
\textbf{Age distribution} \\
\quad 15–24 & 0.11 & 0.12 & 0.01 \\
\quad 25–44 & 0.33 & 0.31 & 0.05 \\
\quad 45–64 & 0.24 & 0.24 & 0.02 \\
\quad 65+ & 0.19 & 0.15 & 0.10 \\
\bottomrule
\end{tabular}
\label{tab:master_balance_pretty}
\end{table}

==> tables/master_balance_table.tex <==
\begin{table}[htbp]
\centering
\small
\begin{tabular}{lccc}
\toprule
Variable & Treated Mean & Control Mean & Abs. Std. diff. \\
\midrule
Rurality: Intermediate & 0.053 & 0.245 & 0.561 \\
Rurality: Rural & 0.000 & 0.330 & 0.992 \\
Rurality: Urban & 0.947 & 0.425 & 1.361 \\
Edu: No education & 0.035 & 0.035 & 0.001 \\
Edu: Mandatory school & 0.174 & 0.197 & 0.060 \\
Edu: Apprenticeship & 0.268 & 0.309 & 0.090 \\
Edu: Maturity & 0.067 & 0.037 & 0.136 \\
Edu: University & 0.097 & 0.045 & 0.201 \\
Edu: Low education & 0.209 & 0.232 & 0.056 \\
Edu: Medium education & 0.335 & 0.346 & 0.022 \\
Edu: High education & 0.097 & 0.045 & 0.201 \\
Socio: Managers & 0.012 & 0.011 & 0.013 \\
Socio: Liberal professions & 0.009 & 0.006 & 0.042 \\
Socio: Other independents & 0.035 & 0.049 & 0.070 \\
Socio: Intellectual/exec. & 0.059 & 0.038 & 0.099 \\
Socio: Intermediate prof. & 0.084 & 0.082 & 0.007 \\
Socio: Qualified non-manual & 0.099 & 0.098 & 0.003 \\
Socio: Qualified manual & 0.027 & 0.044 & 0.092 \\
Socio: Unqualified workers & 0.057 & 0.063 & 0.027 \\
Socio: Active (unattributed) & 0.138 & 0.128 & 0.031 \\
Socio: Unemployed & 0.032 & 0.019 & 0.078 \\
Socio: Inactive & 0.318 & 0.285 & 0.072 \\
Socio: Under 15 & 0.131 & 0.178 & 0.130 \\
Demo: Female share & 0.528 & 0.508 & 0.039 \\
Demo: Swiss share & 0.729 & 0.825 & 0.233 \\
Age: 0–4 & 0.044 & 0.055 & 0.049 \\
Age: 5–14 & 0.087 & 0.124 & 0.119 \\
Age: 15–24 & 0.114 & 0.118 & 0.012 \\
Age: 25–44 & 0.330 & 0.309 & 0.047 \\
Age: 45–64 & 0.238 & 0.245 & 0.016 \\
Age: 65+ & 0.186 & 0.150 & 0.096 \\
\bottomrule
\end{tabular}
\caption{Combined balance table across rurality, education, socio-professional, demographics, and age shares (treated vs control MedStat regions).}
\label{tab:master_balance}
\end{table}


==> tables/overal_att_across_est.tex <==
\begin{table}[H]
\centering
\caption{Overall ATT Across Estimators, 5\,km Buffer}
\label{tab:att_comparison}
\begin{tabular}{lcc}
\toprule
Estimator & ATT & SE \\
\midrule
CS-DR \citep{CALLAWAY2021200}          & $-0.034$ & $(0.298)$ \\
Sun \& Abraham \citep{SUN2021}         & $-0.027$ & $(0.295)$ \\
Stacked DiD \citep{stacked_did} & $-0.175^{***}$ & $(0.038)$ \\
Synthetic DiD \citep{arkhangelsky2021synthetic} & $-0.091$ & $(0.210)$\\
\bottomrule
\end{tabular}
\vspace{0.3cm}
\begin{minipage}{\linewidth}
\setstretch{0.9}
\raggedright
\footnotesize{\textit{Note:} The table reports the pooled ATT averaged
across all post-treatment periods and cohorts for each estimator.
All specifications use the 5\,km buffer and never-treated control
regions. The CS-DR estimator uses a universal base period. The
stacked DiD uses cohort-specific stacks with event-level fixed
effects and both never-treated and not-yet-treated controls.
Synthetic DiD standard errors are obtained via placebo permutation
bootstrap (200 replications). All point estimates are negative,
indicating a reduction in drug-related hospitalization rates
following DCR openings. Standard errors in parentheses.
Significance: $^{***}p<0.01$, $^{**}p<0.05$, $^{*}p<0.10$.}
\end{minipage}
\end{table}


==> tables/pretreat_outcome_balance.tex <==
\begin{table}[H]
\centering
\small
\begin{tabular}{lccc}
\toprule
\textbf{Outcome} & \textbf{Treated Mean} & \textbf{Control Mean} & \textbf{Abs. Std. diff.} \\
\midrule
Overall Outcome & 0.0335 & 0.0211 & 0.0761 \\
Accidental Poisoning & 0.0001 & 0.0000 & 0.0073 \\
Narcotics/Psychodysleptics & 0.0005 & 0.0004 & 0.0067 \\
Mental/Behavioral Disorders & 0.0280 & 0.0174 & 0.0710 \\
HIV & 0.0018 & 0.0013 & 0.0152 \\
Hepatitis & 0.0046 & 0.0031 & 0.0235 \\
\bottomrule
\end{tabular}
\caption{Pre-treatment outcome incidence by group. Entries are means (proportions) and absolute standardized differences.}
\label{tab:pretreat_outcome_balance}
\end{table}

==> tables/pretreatment_balance_abs_smd.tex <==
\begin{table}[H]
\caption{Pre-treatment balance of baseline characteristics (ages 15-74)}
\centering
\tiny
% ↓ reduce vertical spacing between rows (default is 1.0)
{\renewcommand{\arraystretch}{0.6} % try 0.9, 0.8, etc.
\begin{tabular}{lccc}
\toprule
 & \textbf{Treated Mean} & \textbf{Control Mean} & \textbf{Abs. Std. diff.} \\
\multicolumn{4}{l}{\textit{Discrete variables}} \\
\hline
\textbf{Sex} \\
\hline
\quad Female & 0.56 & 0.54 & 1.61 \\
\addlinespace
\hline
\textbf{Age group (5-year)} \\
\hline
\quad 15-19 & 0.03 & 0.04 & 0.28 \\
\quad 20-24 & 0.05 & 0.05 & 0.33 \\
\quad 25-29 & 0.07 & 0.07 & 0.40 \\
\quad 30-34 & 0.09 & 0.09 & 0.45 \\
\quad 35-39 & 0.08 & 0.08 & 0.43 \\
\quad 40-44 & 0.07 & 0.08 & 0.41 \\
\quad 45-49 & 0.08 & 0.08 & 0.42 \\
\quad 50-54 & 0.09 & 0.09 & 0.45 \\
\quad 55-59 & 0.10 & 0.10 & 0.46 \\
\quad 60-64 & 0.10 & 0.10 & 0.48 \\
\quad 65-69 & 0.11 & 0.11 & 0.50 \\
\quad 70-74 & 0.13 & 0.11 & 0.54 \\
\addlinespace
\hline
\textbf{Nationality} \\
\hline
\quad Non-Swiss & 0.27 & 0.22 & 0.77 \\
\quad Swiss & 0.73 & 0.78 & 2.70 \\
\addlinespace
\hline
\textbf{Mode of admission} \\
\hline
\quad Emergency (within 12h) & 0.34 & 0.36 & 1.05 \\
\quad Internal Transfer & 0.01 & 0.00 & 0.13 \\
\quad Other & 0.01 & 0.01 & 0.13 \\
\quad Scheduled / Planned & 0.62 & 0.62 & 1.81 \\
\quad Transfer within 24h & 0.00 & 0.00 & 0.08 \\
\quad Unknown & 0.02 & 0.02 & 0.23 \\
\addlinespace
\hline
\textbf{Stay before admission} \\
\hline
\quad Acute Care (Same) & 0.00 & 0.00 & 0.03 \\
\quad Home & 0.87 & 0.88 & 3.85 \\
\quad Home w/ Home Care & 0.00 & 0.00 & 0.08 \\
\quad Medical Non-Hospital Facility & 0.00 & 0.00 & 0.09 \\
\quad Non-Med. Non-Hosp. Facility & 0.01 & 0.01 & 0.11 \\
\quad Other & 0.02 & 0.02 & 0.19 \\
\quad Other Hospital / Birth Home & 0.07 & 0.06 & 0.39 \\
\quad Penal Institution & 0.00 & 0.00 & 0.05 \\
\quad Psych. Clinic (Same) & 0.00 & 0.00 & 0.01 \\
\quad Psych. Clinic, Other & 0.01 & 0.00 & 0.11 \\
\quad Rehab Clinic (Other) & 0.00 & 0.00 & 0.01 \\
\quad Rehab Clinic (Same) & 0.00 & 0.00 & 0.01 \\
\quad Unknown & 0.02 & 0.02 & 0.22 \\
\addlinespace
\hline
\textbf{Type of care} \\
\hline
\quad Inpatient (Hospitalisation) & 0.87 & 0.91 & 4.50 \\
\quad Outpatient (Ambulatory) & 0.00 & 0.01 & 0.11 \\
\quad Semi-hospitalization (Deprecated) & 0.12 & 0.08 & 0.53 \\
\quad Unknown & 0.00 & 0.00 & 0.02 \\
\addlinespace
\hline
\textbf{Discharge decision} \\
\hline
\quad By Patient (Against Advice) & 0.01 & 0.02 & 0.22 \\
\quad By Third Party & 0.00 & 0.00 & 0.05 \\
\quad By Treating Physician & 0.90 & 0.90 & 4.26 \\
\quad Deceased & 0.01 & 0.01 & 0.16 \\
\quad Internal Transfer & 0.01 & 0.00 & 0.13 \\
\quad Other & 0.01 & 0.01 & 0.17 \\
\quad Unknown & 0.05 & 0.05 & 0.33 \\
\addlinespace
\hline
\textbf{Stay after discharge} \\
\hline
\quad Acute Care Division (Same) & 0.00 & 0.00 & 0.01 \\
\quad Deceased & 0.01 & 0.01 & 0.16 \\
\quad Home & 0.85 & 0.85 & 3.40 \\
\quad Medical Non-Hospital Facility & 0.01 & 0.01 & 0.14 \\
\quad Non-Med. Non-Hosp. Facility & 0.01 & 0.01 & 0.14 \\
\quad Other & 0.01 & 0.01 & 0.15 \\
\quad Other Hospital / Birth Home & 0.04 & 0.03 & 0.27 \\
\quad Penal Institution & 0.00 & 0.00 & 0.04 \\
\quad Psych. Division (Same) & 0.00 & 0.00 & 0.01 \\
\quad Psych. Institution, Other & 0.01 & 0.01 & 0.17 \\
\quad Rehab Division (Same) & 0.00 & 0.00 & 0.02 \\
\quad Rehab Institution, Other & 0.03 & 0.02 & 0.24 \\
\quad Unknown & 0.03 & 0.05 & 0.31 \\
\addlinespace
\hline
\textbf{Post-discharge care} \\
\hline
\quad Deceased & 0.01 & 0.01 & 0.16 \\
\quad Home Care & 0.02 & 0.02 & 0.19 \\
\quad Inpatient Care & 0.05 & 0.05 & 0.33 \\
\quad Other & 0.04 & 0.03 & 0.31 \\
\quad Outpatient Treatment & 0.35 & 0.42 & 1.19 \\
\quad Recovered, No Follow-up & 0.40 & 0.38 & 1.16 \\
\quad Rehabilitation & 0.03 & 0.02 & 0.24 \\
\quad Unknown & 0.09 & 0.08 & 0.45 \\
\midrule
\textbf{N} & 537'872 & 16'110'360 & \\
\end{tabular}
\vspace{0.5cm}
\\
\raggedright 
\footnotesize \textit{Note:} Entries are group shares and absolute standardized differences. The treated group includes individuals residing in areas with a Drug Consumption Room (DCR) prior to treatment, while the control group includes individuals residing in areas without a DCR.
}
\label{tab:pretreat_balance_1}
\end{table}


==> tables/tab_cohort_att.tex <==
\begin{table}[H]
\centering
\caption{Cohort-Specific Average Treatment Effects on the Treated}
\label{tab:cohort_att}
\begin{tabular}{llccc}
\toprule
Cohort & City & 1\,km & 3\,km & 5\,km \\
\midrule
2001 & Geneva/Bern & 0.262*** & 0.244 & 0.142 \\
 & & (0.072) & (0.530) & (0.465) \\
 & & 29.9\% & 27.7\% & 15.2\% \\
\addlinespace
2008 & Lucerne & -1.353*** & -0.506 & -0.585* \\
 & & (0.103) & (0.455) & (0.330) \\
 & & -74.1\% & -39.7\% & -44.3\% \\
\addlinespace
2013 & Basel-Stadt & -0.150*** & -0.150*** & -0.150*** \\
 & & (0.022) & (0.022) & (0.022) \\
 & & -13.9\% & -13.9\% & -13.9\% \\
\addlinespace
2018 & Vaud & 0.142*** & 0.071 & -0.093 \\
 & & (0.019) & (0.072) & (0.136) \\
 & & 15.2\% & 7.4\% & -8.9\% \\
\addlinespace
\midrule
\multicolumn{2}{l}{Treated regions} \\
 & Geneva/Bern & 2 & 12 & 19 \\
 & Lucerne & 1 & 7 & 9 \\
 & Basel-Stadt & 1 & 1 & 1 \\
 & Vaud & 1 & 9 & 11 \\
\midrule
\multicolumn{2}{l}{Control regions} & 608 & 608 & 608 \\
\bottomrule
\end{tabular}
\vspace{0.3cm}
\begin{minipage}{\linewidth}
\setstretch{0.9}
\raggedright
\footnotesize{\textit{Note:} The table reports cohort-specific ATTs
from the doubly robust Callaway \& Sant'Anna (2021) estimator with
never-treated controls and a universal base period. Each cohort
corresponds to the canton(s) where a DCR opened in the indicated year.
The ATT for each cohort is averaged over all available post-treatment
periods. Columns correspond to the geographic buffer used to define
treated Medstat regions. The 2013 cohort (Basel-Stadt) consists of a
single Medstat region (BS02), which falls within all three buffer
zones; the identical point estimate across columns therefore reflects
sample composition rather than an independent geographic robustness
check. The 1\,km estimates for all cohorts are each identified from a
single treated region and should be interpreted with caution. The 2001
cohort (Geneva/Bern) is subject to a limited pre-treatment window of
three years (1998--2000) and a confounding hospitalization surge in
2008; its positive ATT is not interpreted as a causal effect. The 2018
cohort (Vaud) has only five post-treatment years (2018--2022), which
may be insufficient to identify the full treatment effect.
Standard errors clustered at the Medstat region level in parentheses.
Significance: $^{***}p<0.01$, $^{**}p<0.05$, $^{*}p<0.10$.}
\end{minipage}
\end{table}


==> tables/tab_cohort_att_BL.tex <==
\begin{table}[H]
\centering
\caption{Cohort-Specific Average Treatment Effects on the Treated}
\label{tab:cohort_att_BL}
\begin{tabular}{llccc}
\toprule
Cohort & City & 1\,km & 3\,km & 5\,km \\
\midrule
\multirow{}{}{2001} & \multirow{}{}{Geneva/Bern} & -0.304 & -0.196 & -0.403 \\
 & & (0.586) & (0.366) & (0.282) \\
 & & -26.2\% & -17.8\% & -33.2\% \\
\addlinespace
\multirow{}{}{2008} & \multirow{}{}{Lucerne} & -1.311*** & -1.339*** & -1.297*** \\
 & & (0.097) & (0.379) & (0.289) \\
 & & -73.0\% & -73.8\% & -72.7\% \\
\addlinespace
\multirow{}{}{2013} & \multirow{}{}{Basel-Stadt/Land} & -0.168*** & -0.066 & -0.062 \\
 & & (0.022) & (0.060) & (0.093) \\
 & & -15.5\% & -6.4\% & -6.0\% \\
\addlinespace
\multirow{}{}{2018} & \multirow{}{}{Vaud} & 0.147*** & 0.172* & 0.149** \\
 & & (0.019) & (0.088) & (0.076) \\
 & & 15.8\% & 18.8\% & 16.1\% \\
\addlinespace
\midrule
\multicolumn{2}{l}{Treated regions} \\
 & Geneva/Bern & 3 & 19 & 25 \\
 & Lucerne & 1 & 4 & 6 \\
 & Basel-Stadt/Land & 2 & 5 & 9 \\
 & Vaud & 1 & 7 & 10 \\
\midrule
\multicolumn{2}{l}{Control regions} & 608 & 608 & 608 \\
\bottomrule
\end{tabular}
\vspace{0.3cm}
\begin{minipage}{\linewidth}
\setstretch{0.9}
\raggedright
\footnotesize{\textit{Note:} The table reports cohort-specific ATTs
from the doubly robust \cite{CALLAWAY2021200} estimator with
never-treated controls and a universal base period. Each cohort
corresponds to the canton(s) where a DCR opened in the indicated year.
The ATT for each cohort is averaged over all available post-treatment
periods. The 1\,km estimates for all cohorts are each
identified from a single treated region and should be interpreted with
caution. Standard errors clustered at the Medstat region level
in parentheses. Significance: $^{***}p<0.01$, $^{**}p<0.05$,
$^{*}p<0.10$.}
\end{minipage}
\end{table}


==> tables/tab_cohort_att_BL_5km.tex <==
\begin{table}[H]
\centering
\caption{Cohort-Specific Average Treatment Effects on the Treated (ATT) -- 5 km Buffer}
\label{tab:cohort_att_5km}

\begin{tabular}{llcc}
\toprule
Cohort & City & ATT & SE \\
\midrule

2001 & Geneva/Bern      & 0.14 & (0.48) \\
2008 & Lucerne          & -0.59 & (0.37) \\
2013 & Basel-Stadt/Land & 0.04 & (0.07) \\
2018 & Lausanne         & -0.09 & (0.13) \\
\midrule

Treated regions & \multicolumn{3}{c}{46} \\
Control regions & \multicolumn{3}{c}{608} \\
Observations    & \multicolumn{3}{c}{16,200} \\
\bottomrule
\end{tabular}

\vspace{0.3cm}

\begin{minipage}{\linewidth}
\setstretch{0.9}
\raggedright
\footnotesize{\textit{Note:} The table reports cohort-specific average treatment effects on the treated (ATT) for the 5 km buffer specification, estimated using the doubly robust Callaway \& Sant’Anna (2021) estimator with never-treated controls and a universal base period. Each cohort corresponds to the region(s) where Drug Consumption Rooms (DCRs) were introduced in the indicated year. The ATT for each cohort is averaged over all post-treatment periods. The outcome is the log drug-related hospitalization rate per 100,000 inhabitants. The treatment is defined using a 5\,km geographic buffer around DCRs to identify treated Medstat regions. The control group consists of 608 never-treated Medstat regions throughout. Regions near DCRs that opened before 1998 (\textit{always-treated}) are excluded. Standard errors clustered at the Medstat region level are reported in parentheses. Significance: $^{***}p<0.01$, $^{**}p<0.05$, $^{*}p<0.10$.}
\end{minipage}
\end{table}

==> tables/tab_cohort_att_urban_inter.tex <==
\begin{table}[H]
\centering
\caption{Cohort-Specific ATT — Sample restricted to urban and intermediate Medstat regions (413 control regions).}
\label{tab:cohort_att_urban_inter}
\begin{tabular}{llccc}
\toprule
Cohort & City & 1\,km & 3\,km & 5\,km \\
\midrule
\multirow{3}{*}{2001} & \multirow{3}{*}{Geneva/Bern} & 0.305*** & 0.288 & 0.069 \\
 & & (0.086) & (0.553) & (0.493) \\
 & & 35.7\% & 33.4\% & 7.1\% \\
\addlinespace
\multirow{3}{*}{2008} & \multirow{3}{*}{Lucerne} & -1.278*** & -0.432 & -0.510 \\
 & & (0.121) & (0.446) & (0.341) \\
 & & -72.1\% & -35.0\% & -40.0\% \\
\addlinespace
\multirow{3}{*}{2013} & \multirow{3}{*}{Basel-Stadt/Land} & -0.120*** & 0.000 & 0.066 \\
 & & (0.020) & (0.069) & (0.073) \\
 & & -11.3\% & 0.0\% & 6.8\% \\
\addlinespace
\multirow{3}{*}{2018} & \multirow{3}{*}{Vaud} & 0.151*** & 0.081 & -0.084 \\
 & & (0.018) & (0.068) & (0.126) \\
 & & 16.3\% & 8.4\% & -8.0\% \\
\addlinespace
\midrule
\multicolumn{2}{l}{Treated regions} \\
 & Geneva/Bern & 2 & 12 & 18 \\
 & Lucerne & 1 & 7 & 9 \\
 & Basel-Stadt/Land & 1 & 4 & 7 \\
 & Vaud & 1 & 9 & 11 \\
\midrule
\multicolumn{2}{l}{Control regions} & 413 & 413 & 413 \\
\bottomrule
\end{tabular}
\vspace{0.3cm}
\begin{minipage}{\linewidth}
\setstretch{0.9}
\raggedright
\footnotesize{\textit{Note:} The table reports cohort-specific ATTs
from the doubly robust Callaway \& Sant'Anna (2021) estimator with
never-treated controls and a universal base period. Sample restricted to urban and intermediate Medstat regions (413 control regions).
Standard errors clustered at the Medstat region level in parentheses.
Significance: $^{***}p<0.01$, $^{**}p<0.05$, $^{*}p<0.10$.}
\end{minipage}
\end{table}


==> tables/tab_cohort_att_urban_only.tex <==
\begin{table}[H]
\centering
\caption{Cohort-Specific ATT — Sample restricted to urban Medstat regions only (288 control regions).}
\label{tab:cohort_att_urban_only}
\begin{tabular}{llccc}
\toprule
Cohort & City & 1\,km & 3\,km & 5\,km \\
\midrule
\multirow{}{2001} & \multirow{}{}{Geneva/Bern} & 0.223** & 0.206 & -0.014 \\
 & & (0.096) & (0.563) & (0.513) \\
 & & 25.0\% & 22.8\% & -1.3\% \\
\addlinespace
\multirow{}{}{2008} & \multirow{}{}{Lucerne} & -1.334*** & -0.102 & -0.102 \\
 & & (0.134) & (0.599) & (0.625) \\
 & & -73.7\% & -9.7\% & -9.7\% \\
\addlinespace
\multirow{}{}{2013} & \multirow{}{}{Basel-Stadt/Land} & -0.117*** & 0.003 & 0.068 \\
 & & (0.020) & (0.068) & (0.072) \\
 & & -11.1\% & 0.3\% & 7.1\% \\
\addlinespace
\multirow{}{}{2018} & \multirow{}{}{Vaud} & 0.161*** & 0.091 & 0.017 \\
 & & (0.020) & (0.076) & (0.104) \\
 & & 17.5\% & 9.5\% & 1.7\% \\
\addlinespace
\midrule
\multicolumn{2}{l}{Treated regions} \\
 & Geneva/Bern & 2 & 12 & 18 \\
 & Lucerne & 1 & 4 & 4 \\
 & Basel-Stadt/Land & 1 & 4 & 7 \\
 & Vaud & 1 & 9 & 10 \\
\midrule
\multicolumn{2}{l}{Control regions} & 288 & 288 & 288 \\
\bottomrule
\end{tabular}
\vspace{0.3cm}
\begin{minipage}{\linewidth}
\setstretch{0.9}
\raggedright
\footnotesize{\textit{Note:} The table reports cohort-specific ATTs
from the doubly robust Callaway \& Sant'Anna (2021) estimator with
never-treated controls and a universal base period. Sample restricted to urban Medstat regions only (288 control regions).
Standard errors clustered at the Medstat region level in parentheses.
Significance: $^{***}p<0.01$, $^{**}p<0.05$, $^{*}p<0.10$.}
\end{minipage}
\end{table}


==> tables/tab_cohort_urban_only_update.tex <==
\begin{table}[H]
\centering
\caption{Cohort-Specific ATT — Sample restricted to urban Medstat regions only (288 control regions).}
\label{tab:cohort_att_urban_only_up}
\begin{tabular}{llccc}
\toprule
Cohort & City & 1\,km & 3\,km & 5\,km \\
\midrule
\multirow{}{2001} & \multirow{}{}{Geneva/Bern} & 0.22** & 0.21 & -0.01 \\
 & & (0.10) & (0.56) & (0.51) \\
\addlinespace
\multirow{}{2008} & \multirow{}{}{Lucerne} & -1.33*** & -0.10 & -0.10 \\
 & & (0.13) & (0.60) & (0.63) \\
\addlinespace
\multirow{}{2013} & \multirow{}{}{Basel-Stadt/Land} & -0.12*** & 0.00 & 0.07 \\
 & & (0.02) & (0.07) & (0.07) \\
\addlinespace
\multirow{}{2018} & \multirow{}{}{Vaud} & 0.16*** & 0.09 & 0.02 \\
 & & (0.02) & (0.08) & (0.10) \\
\addlinespace
\midrule
\multicolumn{2}{l}{Treated regions} \\
 & Geneva/Bern & 2 & 12 & 18 \\
 & Lucerne & 1 & 4 & 4 \\
 & Basel-Stadt/Land & 1 & 4 & 7 \\
 & Vaud & 1 & 9 & 10 \\
\midrule
\multicolumn{2}{l}{Control regions} & 288 & 288 & 288 \\
\bottomrule
\end{tabular}
\vspace{0.3cm}
\begin{minipage}{\linewidth}
\setstretch{0.9}
\raggedright
\footnotesize{\textit{Note:} The table reports cohort-specific ATTs
from the doubly robust Callaway \& Sant'Anna (2021) estimator with
never-treated controls and a universal base period. Sample restricted to urban Medstat regions only (288 control regions).
Standard errors clustered at the Medstat region level in parentheses.
Significance: $^{***}p<0.01$, $^{**}p<0.05$, $^{*}p<0.10$.}
\end{minipage}
\end{table}

==> tables/tab_matched_cs_att.tex <==
\begin{table}[H]
\centering
\caption{CS-DR ATT: Unconditional, PS-Trimmed, and Covariate-Adjusted, 5\,km}
\label{tab:matched_cs}
\begin{tabular}{llccc}
\toprule
 & & Unconditional & PS-trimmed & With covariates \\
\midrule
\multicolumn{2}{l}{\textit{Overall ATT}} \\
 & ATT & -0.034 & 0.117 & 0.307 \\
 & & (0.299) & (0.328) & (0.542) \\
 & \% change & -3.3\% & 12.4\% & 35.9\% \\
\midrule
\multicolumn{2}{l}{\textit{Cohort ATT}} \\
\multirow{2}{*}{2001} & \multirow{2}{*}{Geneva/Bern} & 0.143 & 0.307 & 0.612 \\
 & & (0.443) & (0.479) & (0.787) \\
\addlinespace
\multirow{2}{*}{2008} & \multirow{2}{*}{Lucerne} & -0.592* & -0.366 & -0.384 \\
 & & (0.357) & (0.368) & (0.443) \\
\addlinespace
\multirow{2}{*}{2013} & \multirow{2}{*}{Basel} & 0.036 & 0.087 & 0.093 \\
 & & (0.072) & (0.069) & (0.069) \\
\addlinespace
\multirow{2}{*}{2018} & \multirow{2}{*}{Vaud} & -0.093 & -0.104 & -0.040 \\
 & & (0.132) & (0.130) & (0.162) \\
\addlinespace
\midrule
Treated regions & & 46 & 46 & 46 \\
Control regions & & 602 & 276 & 587 \\
\bottomrule
\end{tabular}
\vspace{0.3cm}
\begin{minipage}{\linewidth}
\setstretch{0.9}
\raggedright
\footnotesize{\textit{Note:} All estimates use the doubly robust
Callaway \& Sant'Anna (2021) estimator with never-treated controls
and a universal base period. \textit{Unconditional}: full never-treated
control pool, no covariate adjustment. \textit{PS-trimmed}: control
pool restricted to regions with propensity score above the 5th percentile
of the treated distribution; propensity scores estimated via logit on
2000 census characteristics (education, occupation, demographics, urban
typology, log population, and mean pre-treatment drug-related
hospitalization rate 1998--2000). Fifteen never-treated regions with
missing 2000 census education variables excluded from PS estimation.
\textit{With covariates}: log population, share higher education, share
unemployed, share aged 25--44, share Swiss-born, and Medstat urban
typology dummies passed to the doubly robust estimator via
\texttt{xformla}; full control pool retained, covariate adjustment
performed internally. A reduced covariate set is used to avoid perfect
separation given small treated cohort sizes. Standard errors clustered
at the Medstat region level.
Significance: $^{***}p<0.01$, $^{**}p<0.05$, $^{*}p<0.10$.}
\end{minipage}
\end{table}


==> tables/tab_overall_att.tex <==
\begin{table}[H]
\centering
\caption{Overall Average Treatment Effect on the Treated (ATT)}
\label{tab:overall_att}
\begin{tabular}{lccc}
\toprule
 & 1\,km & 3\,km & 5\,km \\
\midrule
ATT & -0.129 & 0.031 & -0.043 \\
    & (0.372) & (0.351) & (0.350) \\
\% change & -12.1\% & 3.1\% & -4.2\% \\
\midrule
Treated regions & 5      & 29     & 40     \\
Control regions & 608    & 608    & 608    \\
Observations    & 15,325 & 15,925 & 16,200 \\
\bottomrule
\end{tabular}
\vspace{0.3cm}
\begin{minipage}{\linewidth}
\setstretch{0.9}
\raggedright
\footnotesize{\textit{Note:} The table reports the overall ATT
estimated using the doubly robust Callaway \& Sant'Anna (2021)
estimator with never-treated controls and a universal base period.
The outcome is the log drug-related hospitalization rate per 100,000
inhabitants. Columns differ in the geographic buffer used to define
treated Medstat regions: 1\,km (5 treated regions), 3\,km (29
treated regions), and 5\,km (40 treated regions). The control group
consists of 608 never-treated Medstat regions throughout. Regions
near DCRs that opened before 1998 (\textit{always-treated}) are
excluded. Standard errors clustered at the Medstat region level in parentheses.
Significance: $^{***}p<0.01$, $^{**}p<0.05$, $^{*}p<0.10$.}
\end{minipage}
\end{table}


==> tables/tab_overall_att_BL_5km.tex <==
\begin{table}[H]
    \centering
    \caption{Overall Average Treatment Effect on the Treated (ATT) -- 5 km Buffer}
    \label{tab:overall_att_5km}
    \begin{tabular}{lcc}
    \toprule
     & ATT & SE \\
    \midrule
    5\,km & -0.03 & (0.31) \\
    \midrule
    Treated regions & \multicolumn{2}{c}{46} \\
    Control regions & \multicolumn{2}{c}{608} \\
    Observations    & \multicolumn{2}{c}{16,200} \\
    \bottomrule
    \end{tabular}
    \vspace{0.3cm}
    \begin{minipage}{\linewidth}
    \setstretch{0.9}
    \raggedright
    \footnotesize{\textit{Note:} The table reports the overall ATT estimated using the doubly robust Callaway \& Sant’Anna (2021) estimator with never-treated controls and a universal base period. The outcome is the log drug-related hospitalization rate per 100,000 inhabitants. The treatment is defined using a 5\,km geographic buffer around DCRs to identify treated Medstat regions. The control group consists of 608 never-treated Medstat regions throughout. Regions near DCRs that opened before 1998 (\textit{always-treated}) are excluded. Standard errors clustered at the Medstat region level are reported in parentheses. Significance: $^{***}p<0.01$, $^{**}p<0.05$, $^{*}p<0.10$.}
    \end{minipage}
\end{table}

==> tables/tab_overall_att_urban_inter.tex <==
\begin{table}[H]
\centering
\caption{Overall ATT — Urban and intermediate Medstat regions only (413 control regions).}
\label{tab:overall_att_urban_inter}
\begin{tabular}{lccc}
\toprule
 & 1\,km & 3\,km & 5\,km \\
\midrule
ATT & -0.084 & 0.076 & -0.064 \\
    & (0.357) & (0.342) & (0.315) \\
\% change & -8.0\% & 7.9\% & -6.2\% \\
\midrule
Treated regions  & 5 & 32 & 45 \\
Control regions  & 413 & 413 & 413 \\
Observations     & 10,450 & 11,125 & 11,450 \\
\bottomrule
\end{tabular}
\vspace{0.3cm}
\begin{minipage}{\linewidth}
\setstretch{0.9}
\raggedright
\footnotesize{\textit{Note:} The table reports the overall ATT estimated
using the doubly robust Callaway \& Sant'Anna (2021) estimator with
never-treated controls and a universal base period. The outcome is the
log drug-related hospitalization rate per 100,000 inhabitants. Urban and intermediate Medstat regions only (413 control regions).
Standard errors clustered at the Medstat region level in parentheses.
Significance: $^{***}p<0.01$, $^{**}p<0.05$, $^{*}p<0.10$.}
\end{minipage}
\end{table}


==> tables/tab_overall_att_urban_inter_5km.tex <==
\begin{table}[H]
\centering
\caption{Overall ATT — Urban and intermediate Medstat regions only (413 control regions), 5\,km buffer.}
\label{tab:overall_att_urban_inter_5km}
\begin{tabular}{lcc}
\toprule
 & ATT & SE \\
\midrule
5\,km & -0.06 & (0.32) \\
\midrule
Treated regions  & 45 \\
Control regions  & 413 \\
Observations     & 11,450 \\
\bottomrule
\end{tabular}
\vspace{0.3cm}
\begin{minipage}{\linewidth}
\setstretch{0.9}
\raggedright
\footnotesize{\textit{Note:} The table reports the overall ATT estimated
using the doubly robust Callaway \& Sant'Anna (2021) estimator with
never-treated controls and a universal base period. The outcome is the
log drug-related hospitalization rate per 100,000 inhabitants. Urban and intermediate Medstat regions only (413 control regions). Standard errors clustered at the Medstat region level in parentheses. Significance: $^{***}p<0.01$, $^{**}p<0.05$, $^{*}p<0.10$.}
\end{minipage}
\end{table}

==> tables/tab_overall_att_urban_only.tex <==
\begin{table}[H]
\centering
\caption{Overall ATT — Urban Medstat regions only (288 control regions).}
\label{tab:overall_att_urban_only}
\begin{tabular}{lccc}
\toprule
 & 1\,km & 3\,km & 5\,km \\
\midrule
ATT & -0.14 & 0.13 & -0.01 \\
SE  & (0.36) & (0.36) & (0.35) \\
\midrule
Treated regions  & 5 & 29 & 39 \\
Control regions  & 288 & 288 & 288 \\
Observations     & 7,325 & 7,925 & 8,175 \\
\bottomrule
\end{tabular}
\vspace{0.3cm}
\begin{minipage}{\linewidth}
\setstretch{0.9}
\raggedright
\footnotesize{\textit{Note:} The table reports the overall ATT estimated
using the doubly robust Callaway \& Sant'Anna (2021) estimator with
never-treated controls and a universal base period. The outcome is the
log drug-related hospitalization rate per 100,000 inhabitants. Urban Medstat regions only (288 control regions). Standard errors clustered at the Medstat region level in parentheses. Significance: $^{***}p<0.01$, $^{**}p<0.05$, $^{*}p<0.10$.}
\end{minipage}
\end{table}

==> tables/tab_overall_att_urban_only_5km.tex <==
\begin{table}[H]
\centering
\caption{Overall ATT — Urban Medstat regions only (288 control regions), 5\,km buffer.}
\label{tab:overall_att_urban_only_5km}
\begin{tabular}{lc}
\toprule
 & 5\,km \\
\midrule
ATT & -0.01 \\
SE  & (0.35) \\
\midrule
Treated regions  & 39 \\
Control regions  & 288 \\
Observations     & 8,175 \\
\bottomrule
\end{tabular}
\vspace{0.3cm}
\begin{minipage}{\linewidth}
\setstretch{0.9}
\raggedright
\footnotesize{\textit{Note:} The table reports the overall ATT estimated
using the doubly robust Callaway \& Sant'Anna (2021) estimator with
never-treated controls and a universal base period. The outcome is the
log drug-related hospitalization rate per 100,000 inhabitants. Urban Medstat regions only (288 control regions). Standard errors clustered at the Medstat region level in parentheses. Significance: $^{***}p<0.01$, $^{**}p<0.05$, $^{*}p<0.10$.}
\end{minipage}
\end{table}

==> tables/tab_sdid_cohort_att.tex <==
\begin{table}[H]
\centering
\caption{Cohort ATT: Callaway \& Sant'Anna vs Synthetic DiD, Within 5\,km}
\label{tab:sdid_comparison}
\begin{tabular}{llcccc}
\toprule
 & & \multicolumn{2}{c}{Callaway \& Sant'Anna}
   & \multicolumn{2}{c}{Synthetic DiD} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
Cohort & City & ATT & SE & ATT & SE \\
\midrule
\multirow{2}{*}{2001} & \multirow{2}{*}{Geneva/Bern} & 0.143 & 0.044 \\
 & & (0.477) & (0.359) \\
\addlinespace
\multirow{2}{*}{2008} & \multirow{2}{*}{Lucerne} & -0.592 & -0.539 \\
 & & (0.370) & (0.738) \\
\addlinespace
\multirow{2}{*}{2013} & \multirow{2}{*}{Basel} & 0.036 & 0.039 \\
 & & (0.070) & (0.155) \\
\addlinespace
\multirow{2}{*}{2018} & \multirow{2}{*}{Vaud} & -0.093 & -0.039 \\
 & & (0.132) & (0.107) \\
\addlinespace
\midrule
\multicolumn{2}{l}{Control regions} &
  \multicolumn{2}{c}{602 never-treated} &
  \multicolumn{2}{c}{602 never-treated} \\
\bottomrule
\end{tabular}
\vspace{0.3cm}
\begin{minipage}{\linewidth}
\setstretch{0.9}
\raggedright
\footnotesize{\textit{Note:} Callaway \& Sant'Anna (2021) estimates
use the doubly robust estimator with never-treated controls and a
universal base period, clustered at the Medstat region level.
Synthetic DiD estimates use the Arkhangelsky et al.\ (2021) estimator
applied cohort-by-cohort, with all 602 never-treated Medstat regions
as the donor pool. SDiD standard errors are obtained via placebo
permutation bootstrap (200 replications). The outcome is the log
drug-related hospitalization rate per 100,000 inhabitants.
The 2001 cohort (Geneva/Bern) is subject to a limited pre-treatment
window and should not be interpreted causally.
Significance: $^{***}p<0.01$, $^{**}p<0.05$, $^{*}p<0.10$.}
\end{minipage}
\end{table}


==> tables/tab_stacked_overall_att.tex <==
\begin{table}[H]
\centering
\caption{Stacked DiD: Overall ATT Across Specifications}
\label{tab:stacked_att}
\begin{tabular}{lcccc}
\toprule
Specification & ATT & SE & \% change & \\
\midrule
5km | both controls | ±5 & -0.175 & (0.038) & -16.0\% & *** \\
3km | both controls | ±5 & -0.143 & (0.047) & -13.3\% & *** \\
\midrule
5km | never-treated | ±5 & -0.178 & (0.038) & -16.3\% & *** \\
3km | never-treated | ±5 & -0.147 & (0.047) & -13.7\% & *** \\
5km | both controls | ±3 & -0.210 & (0.044) & -18.9\% & *** \\
3km | both controls | ±3 & -0.177 & (0.056) & -16.2\% & *** \\
\bottomrule
\end{tabular}
\vspace{0.3cm}
\begin{minipage}{\linewidth}
\setstretch{0.9}
\raggedright
\footnotesize{\textit{Note:} Each row reports the average post-treatment
ATT from a stacked difference-in-differences regression. For each treatment
cohort, a cohort-specific stack is constructed containing the treated regions
within the specified buffer and a clean control group (never-treated regions,
and not-yet-treated regions whose treatment year falls outside the event window
of the focal cohort). All stacks are pooled and estimated jointly with
cohort $\times$ unit and cohort $\times$ year fixed effects. The event-study
interaction terms are \texttt{i(rel\_period, treated, ref=-1)}, with relative
period normalized to zero at $t=-1$. The overall ATT is the simple average of
post-treatment event-study coefficients ($\ell \geq 0$). Standard errors
clustered at the Medstat region level. Main specification: 5\,km buffer,
never-treated and not-yet-treated controls, $\pm 5$ window.
Significance: $^{***}p<0.01$, $^{**}p<0.05$, $^{*}p<0.10$.}
\end{minipage}
\end{table}


==> tables/tab_sub_cohort_att.tex <==
\begin{table}[H]
\centering
\caption{Cohort-Specific ATT by Outcome Category, Within 5\,km}
\label{tab:sub_cohort_att}
\begin{tabular}{llccccc}
\toprule
Cohort & City & Drug-rel. & Mental/Beh. & Hepatitis & HIV & Narcotics \\
\midrule
2001 & Geneva/Bern & \shortstack{-0.403 \\\\ (0.287)} & \shortstack{-0.121 \\\\ (0.236)} & \shortstack{-0.325 \\\\ (0.291)} & \shortstack{-0.446 \\\\ (0.325)} & \shortstack{-0.462 \\\\ (0.397)} \\
\addlinespace
2008 & Lucerne & \shortstack{-1.297*** \\\\ (0.294)} & \shortstack{-0.715*** \\\\ (0.277)} & \shortstack{-1.309*** \\\\ (0.326)} & \shortstack{-0.805** \\\\ (0.391)} & \shortstack{0.364 \\\\ (0.559)} \\
\addlinespace
2013 & Basel & \shortstack{-0.062 \\\\ (0.091)} & \shortstack{-0.084 \\\\ (0.094)} & \shortstack{-0.119 \\\\ (0.110)} & \shortstack{-0.040 \\\\ (0.332)} & \shortstack{-0.365 \\\\ (0.454)} \\
\addlinespace
2018 & Vaud & \shortstack{0.149** \\\\ (0.076)} & \shortstack{0.138** \\\\ (0.070)} & \shortstack{0.212** \\\\ (0.092)} & \shortstack{0.087 \\\\ (0.316)} & \shortstack{-0.220 \\\\ (0.444)} \\
\addlinespace
\midrule
\multicolumn{2}{l}{Control regions} &
  \multicolumn{5}{c}{608 never-treated} \\
\bottomrule
\end{tabular}
\vspace{0.3cm}
\begin{minipage}{\linewidth}
\setstretch{0.9}
\raggedright
\footnotesize{\textit{Note:} Cohort-specific ATTs from the doubly
robust Callaway \& Sant'Anna (2021) estimator, within 5\,km buffer,
never-treated controls, universal base period. Each ATT is averaged
over all available post-treatment periods for the given cohort.
The 2001 cohort (Geneva/Bern) is subject to a limited pre-treatment
window and should be interpreted with caution. The 2018 cohort (Vaud)
has only five post-treatment years. Standard errors clustered at the
Medstat region level in parentheses.
Significance: $^{***}p<0.01$, $^{**}p<0.05$, $^{*}p<0.10$.}
\end{minipage}
\end{table}


Table~\ref{tab:sub_cohort_att} breaks the cohort-specific estimates down by 
diagnostic category. The Lucerne 2008 cohort shows large, statistically 
significant reductions across Drug-related, Mental/Behavioral, Hepatitis, and HIV hospitalizations, confirming that its overall negative effect is not confined to a single outcome type. Narcotics is the exception. The Lucerne point estimate is positive, though imprecise. The Vaud 2018 cohort shows positive and significant 
estimates for Drug-related, Mental/Behavioral, and Hepatitis outcomes
suggesting the short post-treatment window affects all categories equally rather than reflecting a category-specific anomaly. Geneva/Bern and Basel estimates are uniformly imprecise. 

==> tables/tab_sub_overall_att_5km.tex <==
\begin{table}[H]
    \centering
    \caption{Overall ATT by Outcome Category (5 km Buffer)}
    \label{tab:sub_overall_att_5km}   
    \begin{tabular}{lcc}
    \toprule
    Outcome & ATT & SE \\
    \midrule  
    Drug-related (total)        & -0.03 & (0.31) \\
    Mental/Behavioral           & -0.04 & (0.30) \\
    Hepatitis                   & -0.24 & (0.26) \\
    HIV                         & -0.22 & (0.29) \\
    Narcotics                   &  0.14 & (0.19) \\
    \midrule  
    Treated regions  & \multicolumn{2}{c}{46} \\
    Control regions  & \multicolumn{2}{c}{608 (never-treated)} \\
    \bottomrule
    \end{tabular}   
    \vspace{0.3cm}   
    \begin{minipage}{\linewidth}
    \setstretch{0.9}
    \raggedright
    \footnotesize{\textit{Note:} Each cell reports the overall ATT from the doubly robust Callaway \& Sant’Anna (2021) estimator with never-treated controls and a universal base period. Outcomes are log hospitalization rates per 100,000 inhabitants. Sub-outcomes include mental and behavioral disorders (F11--F19), viral hepatitis (B15--B19), HIV disease (B20--B24), and narcotics/psychodysleptics (T40). The treatment is defined using a 5 km geographic buffer around Drug Consumption Rooms (DCRs). Regions near DCRs that opened before 1998 are excluded. Standard errors are clustered at the Medstat region level.}
    \end{minipage}
\end{table}

==> tables/tables_treatment_cohorts_merged.tex <==
\begin{table}[htbp]
\centering
\caption{Adoption of Drug Consumption Rooms by Year, Canton, and MedStat Region}
\label{tab:dcr_adoption}
\begin{threeparttable}
\begin{tabular}{llllll}
\toprule
Year & Canton & City & Acronym & MedStat & Treatment status \\
\midrule
1986 & Bern & Bern & BE & BE02 & Always-treated \\
1992 & Zurich & Zurich & ZH & ZH01 & Always-treated \\
1993 & Solothurn & Solothurn & SO & SO19 & Always-treated \\
1994 & Schaffhausen & Schaffhausen & SH & SH01 & Always-treated \\
1995 & Solothurn & Olten & SO & SO07 & Always-treated \\
\midrule
2001 & Bern & Biel & BE & BE32 & $g=2001$ \\
2001 & Geneva & Geneva & GE & GE01 & $g=2001$ \\
2008 & Lucerne & Lucerne & LU & LU03 & $g=2008$ \\
2013 & Basel-Stadt & Basel & BS & BS02 & $g=2013$ \\
2018 & Vaud & Lausanne & VD & VD03 & $g=2018$ \\
\bottomrule
\end{tabular}
\begin{tablenotes}
\small
\item \textit{Notes:} The table lists the first year a Drug Consumption Room (DCR) opened in each city, along with the corresponding canton and MedStat region code used in the analysis. Facilities that opened before 1998, the first year of the hospitalization panel, are classified as always-treated and excluded from estimation. The remaining five openings define the treatment cohorts $g$ used in the Callaway and Sant'Anna estimator.
\end{tablenotes}
\end{threeparttable}
\end{table}
